Strategies for Tracking Individual IP Packets Towards DDoS

The identification of the exact path that packets are routed in the network is quite a challenge. This paper presents a novel, efficient traceback strategy in combination with a defence system against distributed denial of service (DDoS) attacks named Tracemax. A single packets can be directly traced over many more hops than the current existing techniques allow. It let good connections pass while bad ones get thwarted. Initiated by the victim the routers in the network cooperate in tracing and become automatically self-organised and self-managed. The novel concept support analyses of packet flows and transmission paths in a network infrastructure. It can effectively reduce the effect of common bandwidth and resource consumption attacks and foster in addition early warning and prevention.

==> content/problem.tex <==
\section{PROBLEM DESCRIPTION}

